Mirror Descent View for Neural Network Quantization

Quantizing large Neural Networks (NN) while maintaining the performance is highly desirable for resource-limited devices due to reduced memory and time complexity. It is usually formulated as a constrained optimization problem and optimized via a modified version of gradient descent. In this work, by interpreting the continuous parameters (unconstrained) as the dual of the quantized ones, we introduce a Mirror Descent (MD) framework for NN quantization. Specifically, we provide conditions on the projections (i.e., mapping from continuous to quantized ones) which would enable us to derive valid mirror maps and in turn the respective MD updates. Furthermore, we present a numerically stable implementation of MD that requires storing an additional set of auxiliary variables (unconstrained), and show that it is strikingly analogous to the Straight Through Estimator (STE) based method which is typically viewed as a "trick" to avoid vanishing gradients issue. Our experiments on CIFAR-10/100, TinyImageNet, and ImageNet classification datasets with VGG-16, ResNet-18, and MobileNetV2 architectures show that our MD variants obtain quantized networks with state-of-the-art performance. Code is available at https://github.com/kartikgupta-at-anu/md-bnn.

==> tables/hyper.tex <==
%%%%%%% hyperparams

\begin{table}[]
\scriptsize
\begin{tabular}{l|ccccc}
\toprule

\multirow{3}{*}{} & \multicolumn{5}{c}{\cifar{-10} with \sresnet{-18}} \\
 & \acrshort{MD}-$\softmax$ & \acrshort{MD}-$\tanh$ & \acrshort{MD}-$\softmax$-\acrshort{S} & \acrshort{MD}-$\tanh$-\acrshort{S} & \acrshort{PQ}* \\
%  & u & w & w & w & w \\
 & Binary & Binary & Ternary & Ternary & Ternary \\
\midrule
learning\_rate & 0.001 & 0.001 & 0.001 & 0.01 & 0.01 \\
lr\_scale & 0.2 & 0.3 & 0.3 & 0.2 & - \\
beta\_scale (ours) or reg\_rate (\acrshort{PQ}) & 1.02 & 1.01 & 1.05 & 1.2 & 0.0001 \\
beta\_scale\_interval & 200 & 100 & 500 & 1000 & - \\
weight\_decay & 0.0 & 0.0 & 0.0 & 0.0 & 0.0001 \\

\midrule

\multirow{3}{*}{} & \multicolumn{5}{c}{\cifar{-100} with \sresnet{-18}} \\
 & \acrshort{MD}-$\softmax$ & \acrshort{MD}-$\tanh$ & \acrshort{MD}-$\softmax$-\acrshort{S} & \acrshort{MD}-$\tanh$-\acrshort{S} & \acrshort{PQ}* \\
%  & u & w & w & w & w \\
 & Binary & Binary & Ternary & Ternary & Ternary \\
\midrule 
learning\_rate & 0.001 & 0.001 & 0.001 & 0.001 & 0.001 \\
lr\_scale & 0.2 & 0.3 & 0.1 & 0.5 & - \\
beta\_scale (ours) or reg\_rate (\acrshort{PQ}) & 1.05 & 1.05 & 1.1 & 1.1 & 0.0001 \\
beta\_scale\_interval & 500 & 500 & 100 & 500 & - \\
weight\_decay & 0.0 & 0.0 & 0.0 & 0.0 & 0.0001 \\

\midrule

\multicolumn{1}{c|}{\multirow{4}{*}{}} & \multicolumn{5}{c}{\cifar{-10} with \svgg{-16}} \\
\multicolumn{1}{c|}{} & \acrshort{MD}-$\softmax$ & \acrshort{MD}-$\tanh$ & \acrshort{MD}-$\softmax$-\acrshort{S} & \acrshort{MD}-$\tanh$-\acrshort{S} & \acrshort{PQ}* \\
% \multicolumn{1}{c|}{} & u & w & w & w & w \\
\multicolumn{1}{c|}{} & Binary & Binary & Ternary & Ternary & Ternary \\
\midrule
learning\_rate & 0.01 & 0.001 & 0.001 & 0.01 & 0.1 \\
lr\_scale & 0.2 & 0.3 & 0.3 & 0.3 & - \\
beta\_scale (ours) or reg\_rate (\acrshort{PQ}) & 1.05 & 1.1 & 1.05 & 1.1 & 0.0001 \\
beta\_scale\_interval & 500 & 1000 & 500 & 1000 & - \\
weight\_decay & 0.0 & 0.0 & 0.0 & 0.0 & 0.0001 \\

\midrule

\multirow{3}{*}{} & \multicolumn{5}{c}{\cifar{-100} with \svgg{-16}} \\
 & \acrshort{MD}-$\softmax$ & \acrshort{MD}-$\tanh$ & \acrshort{MD}-$\softmax$-\acrshort{S} & \acrshort{MD}-$\tanh$-\acrshort{S} & \acrshort{PQ}* \\
%  & u & w & w & w & w \\
 & Binary & Binary & Ternary & Ternary & Ternary \\
\midrule
learning\_rate & 0.001 & 0.001 & 0.0001 & 0.001 & 0.0001 \\
lr\_scale & 0.3 & 0.3 & 0.3 & 0.5 & - \\
beta\_scale (ours) or reg\_rate (\acrshort{PQ}) & 1.01 & 1.05 & 1.05 & 1.1 & 0.0001 \\
beta\_scale\_interval & 100 & 500 & 100 & 500 & - \\
weight\_decay & 0.0 & 0.0 & 0.0 & 0.0 & 0.0001 \\

\midrule

\multirow{3}{*}{} & \multicolumn{5}{c}{\tinyimagenet{} with \sresnet{-18}} \\
& \acrshort{MD}-$\softmax$ & \acrshort{MD}-$\tanh$ & \acrshort{MD}-$\softmax$-\acrshort{S} & \acrshort{MD}-$\tanh$-\acrshort{S} & \acrshort{PQ}* \\
% \multicolumn{1}{c|}{} & u & w & w & w & w \\
 & Binary & Binary & Ternary & Ternary & Ternary \\
\midrule

learning\_rate & 0.001 & 0.001 & 0.001 & 0.01 & 0.01 \\
lr\_scale & 0.2 & 0.5 & 0.1 & 0.1 & - \\
beta\_scale (ours) or reg\_rate (\acrshort{PQ}) & 1.02 & 1.2 & 1.2 & 1.2 & 0.0001 \\
beta\_scale\_interval & 200 & 2000 & 500 & 2000 & - \\
weight\_decay & 0.0 & 0.0 & 0.0 & 0.0 & 0.0001 \\

\bottomrule
\end{tabular}
\vspace{1ex}
    \caption{\em Hyperparameter settings used for the experiments. 
	Here, the learning rate is multiplied by {\em lr\_scale} after every {\em lr\_scale\_interval} iterations and annealing hyperparameter $(\beta)$ is multiplied by {\em beta\_scale} after every {\em beta\_scale\_interval} iterations. 
	\kartik{tell about optimizer, lrs interval} }
    \label{tab:hyper1}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
\begin{table}[]
\footnotesize
\begin{tabular}{l|ccccc}
\toprule

\multirow{3}{*}{} & \multicolumn{5}{c}{\cifar{-10} with \sresnet{-18}} \\
 & \acrshort{MD}-$\softmax$-\acrshort{S} & \acrshort{MD}-$\tanh$-\acrshort{S} & \acrshort{GD}-$\tanh$ & \acrshort{PMF}* & \acrshort{PQ} \\
%  & u & w & w & w & w \\
 & Binary & Binary & Binary & Binary & Binary \\
\midrule
learning\_rate & 0.001 & 0.001 & 0.001 & 0.001 & 0.01 \\
lr\_scale & 0.3 & 0.3 & 0.3 & 0.3 & 0.5 \\
beta\_scale (ours) or reg\_rate (\acrshort{PQ}) & 1.02 & 1.02 & 1.1 & 1.1 & 0.0001 \\
beta\_scale\_interval & 200 & 200 & 1000 & 1000 & - \\
weight\_decay & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\

\midrule

\multirow{3}{*}{} & \multicolumn{5}{c}{\cifar{-100} with \sresnet{-18}} \\
 & \acrshort{MD}-$\softmax$-\acrshort{S} & \acrshort{MD}-$\tanh$-\acrshort{S} & \acrshort{GD}-$\tanh$ & \acrshort{PMF}* & \acrshort{PQ} \\
%  & u & w & w & w & w \\
 & Binary & Binary & Binary & Binary & Binary \\
\midrule 
learning\_rate & 0.001 & 0.001 & 0.001 & 0.001 & 0.1 \\
lr\_scale & 0.2 & 0.2 & 0.5 & 0.3 & - \\
beta\_scale (ours) or reg\_rate (\acrshort{PQ}) & 1.1 & 1.2 & 1.01 & 1.01 & 0.001 \\
beta\_scale\_interval & 200 & 500 & 100 & 100 & - \\
weight\_decay & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\

\midrule

\multicolumn{1}{c|}{\multirow{4}{*}{}} & \multicolumn{5}{c}{\cifar{-10} with \svgg{-16}} \\
\multicolumn{1}{c|}{}  & \acrshort{MD}-$\softmax$-\acrshort{S} & \acrshort{MD}-$\tanh$-\acrshort{S} & \acrshort{GD}-$\tanh$ & \acrshort{PMF}* & \acrshort{PQ} \\

%  & u & w & w & w & w \\
 & Binary & Binary & Binary & Binary & Binary \\
\midrule
learning\_rate & 0.001 & 0.001 & 0.001 & 0.001 & 0.01 \\
lr\_scale & 0.3 & 0.2 & 0.3 & 0.5 & 0.5 \\
beta\_scale (ours) or reg\_rate (\acrshort{PQ}) & 1.2 & 1.2 & 1.1 & 1.05 & 0.0001 \\
beta\_scale\_interval & 2000 & 2000 & 1000 & 500 & - \\
weight\_decay & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\

\midrule


\multicolumn{1}{c|}{\multirow{4}{*}{}} & \multicolumn{5}{c}{\cifar{-100} with \svgg{-16}} \\
 & \acrshort{MD}-$\softmax$-\acrshort{S} & \acrshort{MD}-$\tanh$-\acrshort{S} & \acrshort{GD}-$\tanh$ & \acrshort{PMF}* & \acrshort{PQ} \\
%  & u & w & w & w & w \\
 & Binary & Binary & Binary & Binary & Binary \\
 
\midrule
learning\_rate & 0.0001 & 0.001 & 0.001 & 0.0001 & 0.01 \\
lr\_scale & 0.2 & 0.5 & 0.5 & 0.5 & 0.5 \\
beta\_scale (ours) or reg\_rate (\acrshort{PQ}) & 1.2 & 1.05 & 1.1 & 1.02 & 0.0001 \\
beta\_scale\_interval & 500 & 500 & 1000 & 200 & - \\
weight\_decay & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\

\midrule

\multirow{3}{*}{} & \multicolumn{5}{c}{\tinyimagenet{} with \sresnet{-18}} \\
 & \acrshort{MD}-$\softmax$-\acrshort{S} & \acrshort{MD}-$\tanh$-\acrshort{S} & \acrshort{GD}-$\tanh$ & \acrshort{PMF}* & \acrshort{PQ} \\
%  & u & w & w & w & w \\
 & Binary & Binary & Binary & Binary & Binary \\
 \midrule

learning\_rate & 0.001 & 0.001 & 0.001 & 0.001 & 0.01 \\
lr\_scale & 0.1 & 0.1 & 0.5 & 0.5 & - \\
beta\_scale (ours) or reg\_rate (\acrshort{PQ}) & 1.02 & 1.2 & 1.01 & 1.01 & 0.0001 \\
beta\_scale\_interval & 100 & 500 & 100 & 100 & - \\
weight\_decay & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 
\\


\bottomrule
\end{tabular}
\vspace{1ex}
    \caption{\em Hyperparameter settings used for the experiments. 
	Here, the learning rate is multiplied by {\em lr\_scale} after every {\em lr\_scale\_interval} iterations and annealing hyperparameter $(\beta)$ is multiplied by {\em beta\_scale} after every {\em beta\_scale\_interval} iterations. 
	}
    \label{tab:hyper2}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[]
\footnotesize
\centering
\begin{tabular}{l|cccc}
\toprule
\multirow{3}{*}{} & \multicolumn{4}{c}{\cifar{-10} with \sresnet{-18}} \\
 & \acrshort{BC} & \acrshort{REF} & \acrshort{PQ} & \acrshort{GD}-$\tanh$ \\
%  & u & w & w & w & w \\
 & Binary & Float & Ternary & Ternary \\
\midrule
learning\_rate & 0.001 & 0.1 & 0.01 & 0.01 \\
lr\_scale & 0.3 & 0.3 & 0.3 & 0.5 \\
beta\_scale (ours) or reg\_rate (\acrshort{PQ}) & - & - & 0.0001 & 1.02 \\
beta\_scale\_interval & - & - & - & 500 \\
weight\_decay & 0.0 & 0.0001 & 0.0 & 0.0 \\

\midrule

\multirow{3}{*}{} & \multicolumn{4}{c}{\cifar{-100} with \sresnet{-18}} \\
 & \acrshort{BC} & \acrshort{REF} & \acrshort{PQ} & \acrshort{GD}-$\tanh$ \\
%  & u & w & w & w & w \\
 & Binary & Float & Ternary & Ternary \\
\midrule
learning\_rate & 0.001 & 0.1 & 0.01 & 0.01 \\
lr\_scale & 0.2 & 0.1 & 0.2 & 0.5 \\
beta\_scale (ours) or reg\_rate (\acrshort{PQ}) & - & - & 0.0001 & 1.02 \\
beta\_scale\_interval & - & - & - & 1000 \\
weight\_decay & 0.0 & 0.0001 & 0.0 & 0.0 \\

\midrule

\multicolumn{1}{c|}{\multirow{3}{*}{}} & \multicolumn{4}{c}{\cifar{-10} with \svgg{-16}} \\
 & \acrshort{BC} & \acrshort{REF} & \acrshort{PQ} & \acrshort{GD}-$\tanh$ \\
%  & u & w & w & w & w \\
 & Binary & Float & Ternary & Ternary \\
\midrule
learning\_rate & 0.0001 & 0.1 & 0.01 & 0.01 \\
lr\_scale & 0.3 & 0.2 & - & 0.3 \\
beta\_scale (ours) or reg\_rate (\acrshort{PQ}) & - & - & 1e-07 & 1.01 \\
beta\_scale\_interval & - & - & - & 500 \\
weight\_decay & 0.0 & 0.0001 & 0.0 & 0.0 \\

\midrule

\multicolumn{1}{c|}{\multirow{3}{*}{}} & \multicolumn{4}{c}{\cifar{-100} with \svgg{-16}} \\
 & \acrshort{BC} & \acrshort{REF} & \acrshort{PQ} & \acrshort{GD}-$\tanh$ \\
%  & u & w & w & w & w \\
 & Binary & Float & Ternary & Ternary \\
\midrule
learning\_rate & 0.0001 & 0.1 & 0.01 & 0.01 \\
lr\_scale & 0.2 & 0.2 & - & 0.2 \\
beta\_scale (ours) or reg\_rate (\acrshort{PQ}) & - & - & 0.0001 & 1.05 \\
beta\_scale\_interval & - & - & - & 2000 \\
weight\_decay & 0.0 & 0.0001 & 0.0 & 0.0 \\

\midrule

\multirow{3}{*}{} & \multicolumn{4}{c}{\tinyimagenet{} with \sresnet{-18}} \\
 & \acrshort{BC} & \acrshort{REF} & \acrshort{PQ} & \acrshort{GD}-$\tanh$ \\
%  & u & w & w & w & w \\
 & Binary & Float & Ternary & Ternary \\
\midrule
learning\_rate & 0.001 & 0.1 & 0.01 & 0.01 \\
lr\_scale & 0.5 & 0.1 & - & 0.5 \\
beta\_scale (ours) or reg\_rate (\acrshort{PQ}) & - & - & 0.01 & 1.05 \\
beta\_scale\_interval & - & - & - & 2000 \\
weight\_decay & 0.0 & 0.0001 & 0.0 & 0.0 \\

\bottomrule
\end{tabular}
\vspace{1ex}
    \caption{\em Hyperparameter settings used for the experiments. 
	Here, the learning rate is multiplied by {\em lr\_scale} after every {\em lr\_scale\_interval} iterations and annealing hyperparameter $(\beta)$ is multiplied by {\em beta\_scale} after every {\em beta\_scale\_interval} iterations. 
	}
    \label{tab:hyper3}
\end{table}



==> tables/mobile-efficient-results.tex <==
%%%%%%% results
\begin{table*}[t]
    \centering
    \small    
    \begin{tabular}{llccccccc}
        \toprule
        &\multirow{2}{*}{Algorithm}   & \multirow{2}{*}{Space} & \multicolumn{2}{c}{\cifar{-10}} & \multicolumn{2}{c}{\cifar{-100}} & \multicolumn{1}{c}{\tinyimagenet{}}\\
         &&  & \smobnet{V2}  & \seffnet{B0}* & \smobnet{V2}  & \seffnet{B0}*   & \smobnet{V2} \\
        \midrule
        &\acrshort{REF} (float) & $\bfw$ & $93.59$ & $82.11$ & $73.97$ & $41.43$ & $55.92$  \\
        &\acrshort{BC}  & $\bfw$ & $86.84$ & $53.84$ & $65.04$ & $36.34$ & $35.73$  \\
        &\acrshort{PMF}  & $\bfu$ & $89.77$ & $84.47$ & $65.64$ & $51.62$ & $46.90$  \\
        \midrule
        
        \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{Ours}}}
        %\cline{2-9}
        % \multirow{2}{*}{Ours}
        &\acrshort{MD}-$\softmax$-\acrshort{S} & $\bfu$ & $88.37$ & $79.68$ & $65.47$ & $48.60$ & $41.03$  \\
        &\acrshort{MD}-$\tanh$-\acrshort{S} & $\bfw$ & $88.80$ & $80.52$ & $64.95$ & $44.50$ & $40.52$  \\

        \bottomrule
    \end{tabular}
    \vspace{1ex}
    \caption{\em Classification accuracies on the test set on latest networks. * Not imagenet pretrained and input size is $32\times32$.}
        
    \label{tab:res_ternary}
\end{table*}

==> tables/res_float_binary.tex <==
%%%%%%% results
\begin{table*}[h]
    \centering
    \small    
    \begin{tabular}{llccccccc}
        \toprule
        &\multirow{2}{*}{Algorithm}   & \multirow{2}{*}{Space} & \multicolumn{2}{c}{\cifar{-10}} & \multicolumn{2}{c}{\cifar{-100}} & \tinyimagenet{}\\
         &&  &  \svgg{-16}  & \sresnet{-18} & \svgg{-16}  & \sresnet{-18}  & \sresnet{-18} \\
        \midrule
        &\acrshort{REF}* (float) & $\bfw$ & $93.33$ & $94.84$ & $71.50$ & $76.31$ & $58.35$\\
        &\acrshort{BC} \citenew{hubara2016binarized} & $\bfw$ & $90.59$ & $92.82$ & $61.08$ & $69.64$  & $51.31$\\
        &\acrshort{PQ} \citenew{bai2018proxquant} & $\bfw$ & $89.71$ & $92.49$ & $56.73$ & $63.06$ & $40.52$ \\ 

        \bottomrule
    \end{tabular}
    \vspace{1ex}
    \caption{\em Classification accuracies on the test set for different methods for binary quantization with bias, batch norm and fully connected layers allowed to be in floating point.}
        
    \label{tab:res_binary_float}
\end{table*}


==> text/hgd.tex <==
\SKIP{
\begin{figure}
\begin{center}
%\includegraphics[width=\linewidth, trim=4.2cm 4.4cm 8.5cm 2.8cm, clip=true,
%page=3]{pmf-figures.pdf}	%trim=[left botm right top]
\includegraphics[width=\linewidth, trim=1cm 6cm 1cm 2cm, clip=true, page=1]{pmf-ste.pdf}	%trim=[left botm right top]
\caption{\em Illustration of \gls{PMF} and \gls{PMF} with \gls{STE}.\NOTE{Probably not needed}}
\label{fig:pmfste}
\end{center}
\end{figure}
}

\section{Unified View of NN Quantization and Hybrid Gradient Descent}\label{sec:hgd}
%So far we have discussed quantization formulations in two different spaces ($\bfw$-space and $\bfu$-space).
%However, in both cases, the optimization is performed via a modified projected gradient descent which we will call \gls{HGD}.
Before formalizing \acrfull{HGD}, we will first give a common form for objective functions~\twoplaineqref{eq:dnnobj}{eq:simobj} as:
\begin{equation}\label{eq:comobj}
\min_{\bfx\in\calX}\ f(\bfx)\ ,
\end{equation}
where $f(\cdot)$ denotes the loss function by abstracting out the dependency on the dataset $\calD$ and $\calX$ denotes the constraint set.
Note that the constraint set would be different depending on the algorithm. 
For instance, for \gls{BC}~\citenew{courbariaux2015binaryconnect} $\calX=\calQ^m$, however, for \gls{PMF}~\citenew{ajanthan2018pmf} $\calX=\calS$.
%Precisely, in the $\bfw$-space $\calX=\conv(\calQ^m)=[q_{\min}, q_{\max}]^m$ and in the $\bfu$-space $\calX=\calS$. 

%Now, we are ready to formalize the {\em hybrid gradient updates} in network quantization algorithms~\citenew{ajanthan2018pmf,courbariaux2015binaryconnect}.
Recall that, the main characteristic of \gls{HGD} is that the gradients computed in the quantized space are used to update the auxiliary variables.
Formally, the \gls{HGD} update for $\eta > 0$ can be written as:
\begin{align}\label{eq:hybridgd}
\tbfx^{k+1} &= \tbfx^k - \eta\,\bfg^k J_P\ ,\\\nonumber
\bfx^{k+1} &= P(\tbfx^{k+1})\ .
\end{align}
Here $\tbfx\in\R^r$ denotes the auxiliary variables, $P$ denotes the projection to the set $\calX$, $\bfg^k\in\partial f(P(\tbfx^k))$, and $J_P$ is the Jacobian of the projection $P$.
It is worth noting that, this above \gls{HGD} update is in fact equivalent to gradient descent on a modified objective function:
\begin{align}\label{eq:hybridcomobj}
\min_{\tbfx}\ &f(P(\tbfx))\ ,\qquad \text{where}\quad
P(\tbfx) \in \calX\ .
\end{align}
This interpretation sheds light on the motivation behind the \gls{HGD} formulation.

\subsection{\acrlong{STE} based \gls{HGD}}

Note that, \acrfull{STE}~\citenew{stehinton} is a popular method to allow backpropagation through (non-differentiable) projections and has been extensively utilized in network quantization~\citenew{courbariaux2015binaryconnect,hubara2017quantized,rastegari2016xnor,yin2018binaryrelax}.
In fact, \gls{STE} is originally developed to approximate the derivative through the $\sign$ function and in that case, it is defined as~\citenew{hubara2017quantized}:
\begin{equation}\label{eq:qsign}
\frac{\partial \sign(\tx)}{\partial \tx} := \I[|\tx| \le 1]\ .
\end{equation} 

However, in this work, we generalize \gls{STE} to any projection and define it as {\em the Jacobian of the projection being the identity}\footnote{This definition of \gls{STE} is sometimes used even for $\sign$ function~\citenew{bai2018proxquant,yin2018binaryrelax}.}.
Therefore, the corresponding \gls{HGD} update with \gls{STE} can be written as:
\begin{align}\label{eq:mdhybridgd}
\tbfx^{k+1} &= \tbfx^k - \eta\,\bfg^k\ ,\\\nonumber
\bfx^{k+1} &= P(\tbfx^{k+1})\in\calX\ .
\end{align}
%where $P$ is the projection to the set $\calX$ and $\bfg^k\in\partial f(\bfx^k)$.
%A figure illustrating the \gls{PMF} algorithm and its \gls{STE} version is given in~\figref{fig:pmfste}.

\paragraph{Examples of \gls{HGD}:}
Here, we provide some existing algorithms as special cases of \gls{HGD}.
\begin{tight_itemize}
\item When $\calX=\calS$ and $P := \softmax_{\beta}$ (where $\beta>0$, $\beta\to \infty$ as $k\to \infty$, and ${\softmax_{\beta}(\tbfx) := \softmax(\beta\tbfx)}$), the \gls{HGD} update~\plaineqref{eq:hybridgd} is exactly the same as that of \gls{PMF}~\citenew{ajanthan2018pmf}.
\item When $\calX = \{-1,1\}^m$, $P:=\sign$, and $J_P$ is approximated as in~\eqref{eq:qsign}, the resulting \gls{HGD} is exactly the same as \gls{BC}~\citenew{courbariaux2015binaryconnect}.
\item \NOTE{anything else?}
\end{tight_itemize}


Note that, in~\eqref{eq:mdhybridgd}, the gradient is computed in the feasible region $\calX$ but it is directly used to update the auxiliary variables $\tbfx$.
This observation hints the connection to mirror descent in which gradients computed in the primal space are used to update the variables in the dual space (refer~\secref{sec:mda}). 
%Here mirror maps are used to map from primal to dual space.
%This relationship of \gls{HGD} and the dual-averaging version of \gls{MDA} was first observed in~\citenew{bai2018proxquant} however the full potential of \gls{MDA} was not explored.
To this end, in the following section we prove under certain conditions on the projection, the \gls{STE} based \gls{HGD} is equivalent to \gls{MD} and provide an analytical method to derive mirror maps given projections. 
 
 
 Neural networks quantization is the process of training a NN such that the learned weights, in the end, are quantized. 
Normally, it is posed as an iterative process where the network benefits from both, the continuous $\Tilde{\bfx}$ and its discrete counterpart $\bfx$ (obtained using a projection $P$), during the training process. 
Given a projection $P:\Tilde{\bfx} \to \bfx$, ideally, the gradient update should be of the following form
\begin{align}
\label{eq:gradUpdateIdeal}
    \Tilde{\bfx}_{t+1} = \Tilde{\bfx}_{t} - \eta \bfg_t \frac{\delta P(\Tilde{\bfx})}{\delta \Tilde{\bfx}}
\end{align}
However, in practice, ignoring $\frac{\delta P(\Tilde{\bfx})}{\delta \Tilde{\bfx}}$, which is equivalent to making it an identity matrix, works very well and has been used vastly in the literature (CITE), leading to the following update
\begin{align}
\label{eq:gradUpdate}
    \Tilde{\bfx}_{t+1} = \Tilde{\bfx}_{t} - \eta \bfg_t 
\end{align}
From the first look of the above update, it does not make much sense as the $\Tilde{\bfx}_t$ is being updated using the gradients computed at $P(\Tilde{\bfx})$ which is completely different from $\Tilde{\bfx}_t$. Here we justify this update by showing that it actually is exactly the same as the very well studied Mirror Descent algorithm. To this end, first of all, we provide theoretical conditions on the projection $P$  that allows the update to be exactly the same as the MD update. Then, we show how tanh and softmax projections actually satisfy these conditions. Finally, we analytically derive the mirror maps, and corresponding updates, for these two projections. 

%In this section, we prove that for certain conditions on the projection, the \gls{STE} based \gls{HGD}~(\eqref{eq:mdhybridgd}) is equivalent to the \gls{MD} algorithm~(\eqref{eq:md1}) and analytically derive the corresponding mirror maps from the projection itself.
%In this section, we will try to derive mirror-maps from projections which would be useful to obtain analogous mirror descent algorithms for network quantization algorithms with different projections.
%Precisely, we will show that for certain projections, the \gls{HGD} with \gls{STE} (\eqref{eq:mdhybridgd}) can be shown to be equivalent to \gls{MDA} (\eqref{eq:md1}) where the corresponding mirror-maps are derived from the projection itself.
Theorem~\ref{thm:mdaproj} presents the conditions required for a projection $P$ for the update~\ref{eq:gradUpdate} to mimic MD update. It mainly states that if $P^{-1}$ is monotonically increasing, then there exist a valid mirror map which can further be used to obtain the MD update steps (refer Section for details). Intuitively, as shown in~\figref{fig:mdaproj}, one can think of the projected point $P(\Tilde{\bfx})$ lying in the primal space, and the gradient through the mirror map in the dual space which is the space of the gradients in the continuous space (notation). Since the mirror map is obtained using the inverse of the projection $P^{-1}$, it naturally leads to the gradients computed at the projected point $P(\Tilde{\bfx})$ but mapped to the dual space. This gradient is then updated in the dual space, which is then projected back into the primal space quantized space, and projected to the feasible set by finding the point that minimizes the Bregman divergence.

\begin{thm}\label{thm:mdaproj}
Let $\calX$ be a compact convex set and $P:\R^r \to \calC$ be an invertible function where $\calC\subset\R^r$ is a convex open set such that $\calX=\bcalC$ ($\bcalC$ denotes the closure of $\calC$).
Now, if $P^{-1}$ satisfy:
\begin{tight_enumerate}
  \item $P^{-1}$ is monotonically increasing.
  %\item $P^{-1}(\calC) = \R^r$.\NOTE{May be not necessary?}
  \item $\lim_{\bfx\to\partial \calC}\|P^{-1}(\bfx)\| = \infty$ ($\partial \calC$ denotes the boundary of $\calC$).
\end{tight_enumerate}
Then, 
\begin{tight_enumerate}
  \item $\Phi(\bfx) = \langle\bfone,\int \iproj(\bfx) d\bfx\rangle$ is a valid mirror map, where $\bfone$ is an $r$-dimensional vector of all ones.
  \item The \gls{STE} based \gls{HGD} update~\plaineqref{eq:mdhybridgd} is equivalent to the \gls{MD} update~\plaineqref{eq:md1} with mirror map ${\Phi(\bfx) = \langle\bfone,\int \iproj(\bfx) d\bfx\rangle}$.
\end{tight_enumerate}
%\NOTE{Check any other conditions (or redundant conditions) on $P$ for $\Phi(\bfw)$ to be a valid mirror-map!}
\end{thm}
\begin{proof}
This can be proved by noting that $\nabla\Phi(\bfx) = \iproj(\bfx)$. Please refer to Appendix~\myref{A}.
\SKIP{
From the fundamental theorem of calculus, the gradient of $\Phi(\bfx)$ satisfies, $\nabla\Phi(\bfx) = \iproj(\bfx)$. Since $\iproj$ is monotonically increasing, $\Phi(\bfx)$ is strictly convex and differentiable.
Now, from the definition of projection and since it is invertible (\ie, $\iproj$ is {\em one-to-one} and {\em onto}), $\nabla\Phi(\calC) = \iproj(\calC) = \R^r$.  
Therefore, together with condition (2), we can conclude that $\Phi(\bfx) = \langle\bfone,\int \iproj(\bfx) d\bfx\rangle$ is a valid mirror map (refer~\dfnref{dfn:mm}).
Now, the \gls{MD} update~\plaineqref{eq:md1} can be written as:
\begin{align}
\iproj(\bfy^{k+1}) &= \iproj(\bfx^k) - \eta\,\bfg^k, \qquad\mbox{where $\bfg^k\in\partial f(\bfx^k)$ and $\bfy^{k+1}\in\calC$}\ ,\\\nonumber
\bfx^{k+1} &= \amin{\bfx\in\primal}\, D_{\Phi}(\bfx, \bfy^{k+1})\ .
\end{align}
Note that, since $\calX=\bcalC$,
\begin{equation}
\bfx^{k+1} = \amin{\bfx\in\primal}\, D_{\Phi}(\bfx, \bfy^{k+1}) = \bfy^{k+1}\ .
\end{equation}
Since, $\iproj(\bfx^k) = \tbfx^k$, and $\iproj(\bfy^{k+1}) = \iproj(\bfx^{k+1}) = \tbfx^{k+1}$, this is exactly the same as~\eqref{eq:mdhybridgd}. Hence, the proof is complete.\NOTE{please verify this}
\NOTE{may be moved to appendix}
}
\end{proof}
 
 
 

==> text/mda_nnq.tex <==
\section{Mirror Descent for NN Quantization}
Even thogh $\tL$ is non-convex,\NOTE{What are we losing due to nonconvexity? Is it still convergent?} we intend to optimize~\eqref{eq:simobj} using \gls{MDA}.

\subsection{Entropic Descent}
To this end, one can easliy see that the primal space is the polytope $\calS$ and a straight-foward choice for the mirror map is the negative entropy~\citenew{bubeck2015convex}.
Precisely, the mirror map
\begin{equation}
\Phi(\bfu) = -H(\bfu) = \sum_{j=1}^m\sum_{\lambda\in\calQ}u_{j:\lambda}\,\log u_{j:\lambda}\ ,
\end{equation}
where $\calC=\R^{md}_{++}$.
Furthermore, the Bregman divergence associated with entropy is the \acrshort{KL}-divergence, \ie, 
\begin{equation}
D_{\Phi}(\bfu,\bfv) = \kl{\bfu}{\bfv} = \sum_{j=1}^m\sum_{\lambda\in\calQ}u_{j:\lambda}\,\log \frac{u_{j:\lambda}}{v_{j:\lambda}}\ .
\end{equation}
When entropy is chosen as the mirror map, the resulting algorithm is usually referred to as \gls{EDA}~\citenew{beck2003mirror} or \gls{EGD}.
In this case, the update takes the following form:
\begin{align}\label{eq:eda}
\bfu^{k+1} &= \amin{\bfu\in\calS}\, \langle \eta\,\bfg^k, \bfu\rangle + \kl{\bfu}{\bfu^k}\ ,\\
u^{k+1}_{j:\lambda} &= \frac{u_{j:\lambda}^k\,e^{-\eta\,g^{k}_{j:\lambda}}}{\sum_{\mu  \in \calQ} \; 
u_{j:\mu}^k\,e^{-\eta\,g^{k}_{j:\mu}}}\quad \forall\, \lambda\in\calQ,\quad \forall\,j\in\allweights \ .
\end{align}
Here, the above equation is simplified by writing the Lagrangian and setting the derivatives with respect to $\bfu$ to zero.
Note that, similar to~\citenew{ajanthan2018pmf}, to gradually enforce a quantized solution one could use an annealing hyperparameter $\beta^k>0$.
In this case, the mirror map is modified at each iteration as:
\begin{equation}
\Phi^k(\bfu) = \frac{-H(\bfu)}{\beta^k}\ ,
\end{equation} 
where $\beta^k\to \infty$ as $k\to \infty$.
\NOTE{not sure on the effect of this in optimization \wrt \gls{MDA}.}
Consequently, the modified \gls{EDA} update can be written as:
\begin{equation}
u^{k+1}_{j:\lambda} = \frac{u_{j:\lambda}^k\,e^{-\eta\,\beta^kg^{k}_{j:\lambda}}}{\sum_{\mu  \in \calQ} \; 
u_{j:\mu}^k\,e^{-\eta\,\beta^kg^{k}_{j:\mu}}}\quad \forall\, \lambda\in\calQ,\quad \forall\,j\in\allweights \ .
\end{equation}
Similarly, the update of the dual averaging version of \gls{EDA} can be written as:
\begin{align}
\bfu^{k+1} &= \amin{\bfu\in\calS}\, \eta \sum_{s=0}^{k}\langle \bfg^s, \bfu\rangle + \Phi^k({\bfu})\ ,\\
\bfu^{k+1} &= \amin{\bfu\in\calS}\, \eta \langle \bbfg^k, \bfu\rangle - \frac{H(\bfu)}{\beta^k}\ ,\quad\mbox{where $\bbfg^k = \sum_{s=0}^{k} \bfg^s$}\ ,\\
u^{k+1}_{j:\lambda} &= \frac{e^{-\eta\,\beta^k\bg^{k}_{j:\lambda}}}{\sum_{\mu  \in \calQ} \; 
e^{-\eta\,\beta^k\bg^{k}_{j:\mu}}}\quad \forall\, \lambda\in\calQ,\quad \forall\,j\in\allweights \ .
\end{align}
Notice the similarity between the above equations and Eqs.~(10)~and~(12) of \gls{PMF}~\citenew{ajanthan2018pmf}.

\NOTE{other mirror maps? or any combinations?, optimization in the $\bfw$ space?}

\subsection{Quadratic Mirror Map}
A standard choice for mirror map is the $L_2$ norm. 
Precisely, 
\begin{equation}
\Phi(\bfu) = \frac{1}{2}\|\bfu\|^2_2\ ,
\end{equation}
where $\calC=\R^{md}$.
The associated Bregman divergence is given by,
 \begin{equation}
D_{\Phi}(\bfu,\bfv) = \frac{1}{2}\|\bfu - \bfv\|_2^2\ .
\end{equation}
Similarly, by introducing $\beta^k$,~\eqref{eq:eda} can now be written as:
\begin{align}\label{eq:qmda}
\bfu^{k+1} &= \amin{\bfu\in\calS}\, \langle \eta\,\bfg^k, \bfu\rangle + \frac{1}{2\beta^k}\|\bfu - \bfu^k\|_2^2\ .
\end{align}
%This is a standard proximal formulation and the above equation can be minimized optimally using the Frank-Wolfe algorithm~\citenew{ajanthan2016efficient,frank1956algorithm,lacoste2012block} or solve the KKT conditions~\citenew{boyd2009convex}. 
%approximately by separating projection from optimization\NOTE{more later, sparsemax \etc}.
%\NOTE{write down the final update equations for binary and think about other quantization levels.}
This can be shown to be equivalent to projected gradient descent~\citenew{bubeck2015convex}. 
In fact, when $\Phi(\bfu) = \frac{1}{2}\|\bfu\|^2_2$, ${\nabla\Phi(\bfu) = \bfu}$, \ie, the mapping from primal to dual is an {\em identity mapping}.



\section{Mirror Descent in the $w$-space}
Note that there is no restriction for \gls{MDA} to be applied in the $w$-space.
In fact, \gls{PQ}~\citenew{bai2018proxquant} first noticed the connection to the dual averaging version of \gls{MDA} and \gls{BC}, however the full potential of \gls{MDA} was not explored.
To this end, we first give a relaxed formulation of \gls{NN} quantization in the $w$-space~(\eqref{eq:dnnobj}) and discuss different choices of mirror-maps.
\begin{align}\label{eq:dnnobjr}
\min_{\bfw} L(\bfw;\calD) &:= \frac{1}{n} \sum_{i=1}^n
\ell(\bfw;(\bfx_i,\bfy_i))\ ,\\\nonumber
\bfw &\in \calT := [q_{\text{min}}, q_{\text{max}}]^m\ , 
\end{align}
where $q_{\text{min}}$ and $q_{\text{max}}$ are the smallest and largest elements in $\calQ$.
Note that, $[q_{\text{min}}, q_{\text{max}}] = \conv({\calQ})$ and $\calT = \conv({\calQ}^m)$.

\subsection{Quadratic Mirror Map}
Let $\Phi(\bfw) = \frac{1}{2}\|\bfw\|^2_2$ where $\calC=\R^{m}$. 
Now the associated Bregman divergence is given by,
 \begin{equation}
D_{\Phi}(\bfw,\bfv) = \frac{1}{2}\|\bfw - \bfv\|_2^2\ .
\end{equation}
Similarly, by introducing $\beta^k$,~\eqref{eq:eda} can now be written as:
\begin{align}\label{eq:qmdaw}
\bfw^{k+1} &= \amin{\bfw\in\calT}\, \langle \eta\,\bfg^k, \bfw\rangle + \frac{1}{2\beta^k}\|\bfw - \bfw^k\|_2^2\ .
\end{align}
%This is a standard proximal formulation and the above equation can be minimized optimally using the Frank-Wolfe algorithm~\citenew{ajanthan2016efficient,frank1956algorithm,lacoste2012block} or solve the KKT conditions~\citenew{boyd2009convex}. 
%approximately by separating projection from optimization\NOTE{more later, sparsemax \etc}.
%Notice, when $\beta^k\to \infty$, $\bfw^{k+1}$ approaches to a discrete solution.
%\NOTE{write down the final update equations for binary and think about other quantization levels.}
This is exactly equivalent to projected gradient descent~\citenew{bubeck2015convex}.

\subsection{Any Mirror-map Corresponding to $\tanh$?}
Note that, in case of binary, \ie, $\calQ=\{-1,1\}$, $\tanh$ is a differentiable way of projecting to the interval $[-1,1]$.
In particular, let $\tw\in\R$, and $\beta>0$ the $\tanh$ projection can be written as:
\begin{equation}\label{eq:tanh}
w = \tanh(\beta\tw) = \frac{e^{2\beta \tw} - 1}{e^{2\beta \tw} + 1}\ .
\end{equation}
It is easy to verify that $w\in[-1,1]$ and $w$ approaches a discrete solution when $\beta\to\infty$.
In fact, $\tanh$ shares many similarities with $\softmax$ (in the $\bfu$-space) and it would be interesting to explore if there is an interpretation for $\tanh$ analogous to the entropy based interpretation of $\softmax$.
%\NOTE{It would be great, if we can come up with a mirror-map, that would have a closed form solution for each \gls{MDA} update resembling $\tanh$!} 



